OccuQuest: Mitigating Occupational Bias for Inclusive Large Language Models

The emergence of large language models (LLMs) has revolutionized natural language processing tasks. However, existing instruction-tuning datasets suffer from occupational bias: the majority of data relates to only a few occupations, which hampers the instruction-tuned LLMs to generate helpful responses to professional queries from practitioners in specific fields. To mitigate this issue and promote occupation-inclusive LLMs, we create an instruction-tuning dataset named \emph{OccuQuest}, which contains 110,000+ prompt-completion pairs and 30,000+ dialogues covering over 1,000 occupations in 26 occupational categories. We systematically request ChatGPT, organizing queries hierarchically based on Occupation, Responsibility, Topic, and Question, to ensure a comprehensive coverage of occupational specialty inquiries. By comparing with three commonly used datasets (Dolly, ShareGPT, and WizardLM), we observe that OccuQuest exhibits a more balanced distribution across occupations. Furthermore, we assemble three test sets for comprehensive evaluation, an occu-test set covering 25 occupational categories, an estate set focusing on real estate, and an occu-quora set containing real-world questions from Quora. We then fine-tune LLaMA on OccuQuest to obtain OccuLLaMA, which significantly outperforms state-of-the-art LLaMA variants (Vicuna, Tulu, and WizardLM) on professional questions in GPT-4 and human evaluations. Notably, on the occu-quora set, OccuLLaMA reaches a high win rate of 86.4\% against WizardLM.

==> fig_tex/fig_different_answers.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/different_answers.resized.pdf}
    \caption{The responses produced by distinct instruction-tuned models in response to an identical query.}
    \label{fig_different_answers}
\end{figure*}

==> fig_tex/tab_benchmarks.tex <==
\begin{table}[ht]
\centering
\caption{Evaluation results on comprehensive benchmarks, with the top-performing results highlighted in \textbf{bold}.}
\label{tab_benchmarks}
\begin{tabular}{lcccc}
    \toprule
    \textbf{Model}   & \textbf{MMLU \tiny{(0 shot)}} & \multicolumn{1}{l}{\textbf{GSM8K \tiny{(8 shot)}}} & \multicolumn{1}{l}{\textbf{BBH \tiny{(cot)}}} & \multicolumn{1}{l}{\textbf{HumanEval \tiny{(P@10)}}} \\ \midrule
    LLaMA-7B         & 30.8          & 9.9           & 32.5          & 16.2          \\
    Vicuna-7B        & 44.4          & 16.1          & 34.6          & 14.8          \\
    Tulu-7B          & 44.4          & 26.8          & \textbf{37.0} & 20.6          \\
    WizardLM-7B      & 36.1          & 14.9          & 31.8          & 20.7          \\
    % OccuLLaMA-7B     & 33.4          & 9.4           & 28.0          & 11.5          \\
    ProLLaMA-7B      & \textbf{46.2} & \textbf{31.2} & 35.5          & \textbf{21.2} \\      \midrule
    LLaMA-13B         & 39.3          & 16.5          & 37.0          & 21.1          \\
    Vicuna-13B        & \textbf{49.2} & 26.2          & 40.8          & 24.9          \\
    Tulu-13B          & \textbf{49.2} & 35.4          & \textbf{43.2} & 23.8          \\
    WizardLM-13B      & 48.9          & 34.0          & 36.6          & \textbf{31.7} \\
    % OccuLLaMA-13B     & 42.7          & 13.2          & 36.5          & 17.0          \\
    ProLLaMA-13B      & \textbf{49.2} & \textbf{36.3} & 39.7          & 23.1           \\ \midrule
    ChatGPT      & 67.9           & 76.0          & 66.1          & 88.4          \\
    GPT-4        & 82.4           & 92.5          & 88.0          & 94.1          \\ \bottomrule
\end{tabular}
\end{table}
